Bayes-Optimal BER and AUC: Estimation and Evaluation of Estimators

A fundamental quantity in machine learning is the optimal performance achievable by any model on a given task. Estimating this quantity allows us to distinguish the irreducible part of the error from a deficiency of the model, telling us how much room for improvement remains. Recent work has shown that the Bayes error, or equivalently the optimal accuracy, can be estimated from soft labels in binary classification. However, accuracy is often a poor summary of performance in settings with severe class imbalance or noisy annotations, where metrics such as the balanced error rate (BER) and the area under the ROC curve (AUC) are more appropriate. We address this gap with two complementary contributions. (i) Estimation. We propose soft-label-based estimators for the optimal BER and AUC. We first consider the clean setting in which true soft labels and the class prior are known, and then extend the estimators to a more realistic setting in which the class prior is unknown and the observed soft labels are corrupted by an unknown order-preserving transformation, possibly followed by additive noise. In the latter setting, we approximately recover the clean soft labels via isotonic regression with auxiliary hard labels, estimate the class prior with a clipped mean of the hard labels, and derive finite-sample error bounds for the resulting plug-in estimators. (ii) Evaluation. Since the optimum is unobservable on real datasets, evaluating any such estimator is itself nontrivial. We extend the FeeBee framework, originally proposed for evaluating Bayes-error estimators, to the optimal BER and AUC. The resulting procedure provides practical evaluation scores without requiring knowledge of the optimum, and applies to any estimator of the optimal BER or AUC, not only our proposed ones. Experiments on synthetic and real-world datasets validate both the estimators and the evaluation procedure.

==> sections/clean/ber-auc/alg-bestauc.tex <==
\subsection{Near-linear time algorithm for computing $\widehat{\bestauc}$}
\label{sec:alg-bestauc}

The definitions of
$\widehat{\bestauc_1}$,
$\widehat{\bestauc_2}$
and
$\widehat{\Delta}_\auc$
involve summation over all pairs of indices $(i, j)$,
so a naive algorithm would take $\Theta(n^{2})$ time
to compute each of them.
This can be a significant bottleneck, or even prohibitive,
for large-scale datasets.
This computational challenge is common for many \emph{U-statistics}
\citep{hoeffding1948class} of degree 2 or higher.
$\widehat{\bestauc_1}$, 
$\widehat{\bestauc_2}$
and
$\widehat{\Delta}_\auc$
are examples of degree-two U-statistics 
and are no exception.
The literature has addressed this challenge typically by
using Monte-Carlo approximation of original U-statistics,
which are called \emph{incomplete U-statistics}
\citep{blom1976some,clemenccon2016scaling,lee2019u}.
This approach reduces the number of terms to be added up and
thus the computational cost, 
but it inevitably introduces additional variance.

\begin{wrapfigure}[11]{r}{0.49\textwidth}
  \vspace{-\intextsep}
  \small
  \hrule height.8pt depth0pt \kern2pt
  \captionof{algorithm}{An efficient algorithm for computing $\widehat{\bestauc_1}$}
  \label{alg:bestauc}
  \kern2pt\hrule\kern2pt
  \begin{algorithmic}
    \INPUT Soft labels $\eta_{1}, \dots, \eta_{n}$, class prior $\theta$
    \STATE $\eta_{(1)}, \dots, \eta_{(n)} \gets$ sort $\eta_{1}, \dots, \eta_{n}$ in ascending order
    \STATE $\mathrm{SUM} \gets 0$
    \STATE $\mathrm{PREFIX} \gets 0$
    \FOR{$j = 2$ \textbf{to} $n$}
      \STATE $\mathrm{PREFIX} \gets \mathrm{PREFIX} + \eta_{(j-1)}$
      \STATE $\mathrm{SUM} \gets \mathrm{SUM}
      + (1 - \eta_{(j)}) \cdot \mathrm{PREFIX}$
    \ENDFOR
    \OUTPUT $1 - \frac{\mathrm{SUM}}{n (n-1) \theta (1-\theta)}$
  \end{algorithmic}
  \kern2pt\hrule\relax
\end{wrapfigure}


Fortunately, however, it turns out that 
$\widehat{\bestauc_1}$, 
$\widehat{\bestauc_2}$
and
$\widehat{\Delta}_\auc$
have special structures that enable efficient computation
without relying on approximation.
For example, 
the exact $\widehat{\bestauc_1}$ can be computed 
in $O(n \log n)$ time
in the worst case
by \cref{alg:bestauc};
the proof is given in \cref{thm:alg-bestauc}.
We also provide $O(n \log n)$-time algorithms 
for exactly computing 
$\widehat{\bestauc_2}$ (\cref{alg:bestauc-max})
and 
$\widehat{\Delta}_\auc$ (\cref{alg:auc-delta-vhat})
in the appendices.







==> sections/clean/ber-auc/bound.tex <==
\subsection{Estimation error bounds}
\label{sec:clean:ber-auc:bound}

Our estimators of the optimal BER and AUC
enjoy the following finite-sample bounds 
on their estimation errors.

\begin{theorem}[store=thm:ber-auc:bound]
  \label{thm:ber-auc:bound}
  For any $\delta > 0$,
  with probability at least $1 - \delta$,
  we have
  $
    \lvert
      \widehat{\bestber}
      -
      \bestber
    \rvert
    \leq
    \sqrt{
      \frac{\log (2/\delta)}{8n}
    }
  $.
\end{theorem}

\begin{theorem}[store=thm:ber-auc:bound:auc:bernstein]
  \label{thm:ber-auc:bound:auc:bernstein}
  For any $\delta > 0$,
  with probability at least $1 - \delta$,
  we have \IfRestatingTF{
    \begin{equation}
      \nonumber
      \abs{
        \widetilde{\bestauc}
        -
        \bestauc
      }
      \leq
      \sqrt{
        \frac{\log (2/\delta)}{\theta (1 - \theta) n}
      }
      \text{.}
    \end{equation}
  }{$
      \lvert
        \widetilde{\bestauc}
        -
        \bestauc
      \rvert
      \leq
      \sqrt{
        \frac{\log (2/\delta)}{\theta (1 - \theta) n}
      }
  $.}
\end{theorem}

\begin{remark}
  \cref{thm:ber-auc:bound}
  simply follows from the Hoeffding bound.
  \cref{thm:ber-auc:bound:auc:bernstein}
  needs a more careful analysis:
  while we can use basic tools like
  Hoeffding's inequality
  \eqref{eq:hoeffding-u-statistic}
  for U-statistics
  or the bounded difference inequality,
  such tools lead to a bound of stochastic order
  $O_p(\frac{1}{ \theta (1 - \theta) \sqrt{n} })$.
  The constant factor $\frac{1}{\theta (1 - \theta)}$
  blows up under severe class imbalance, i.e., 
  when $\theta$ is close to $0$ or $1$.
  We instead employ the Bernstein-type inequality
  \eqref{eq:bernstein-u-statistic}
  for U-statistics
  to improve the $\theta$-dependence
  to $\frac{1}{\sqrt{\theta (1 - \theta)}}$,
  resulting in the bound in
  \cref{thm:ber-auc:bound:auc:bernstein}.
  See \cref{sec:proof-clean:bound}
  for details.
\end{remark}


==> sections/clean/ber-auc/min-vs-max.tex <==
\subsection{Unbiased estimators: Min formula vs. max formula}
\label{sec:min-vs-max}

In \cref{lem:bestber},
we saw that the best possible BER can be 
expressed in two different ways:
$\bestber = \E{\phimin_{\ber}(\eta(x))} = \E{\phimax_{\ber}(\eta(x))}$.
This naturally leads to two different 
unbiased estimators of $\bestber$:
$
  \widehat{\bestber_1} 
  \coloneqq
  \frac{1}{n} \sum_{i=1}^n \phimin_{\ber}(\eta_{i})
$
and
$
  \widehat{\bestber_2} 
  \coloneqq
  \frac{1}{n} \sum_{i=1}^n \phimax_{\ber}(\eta_{i})
$.
We call $\widehat{\bestber_1}$ 
the \emph{min formula} for BER
because $\phimin_{\ber}$ uses the $\min$ operation,
and $\widehat{\bestber_2}$
the \emph{max formula}
because $\phimax_{\ber}$ uses the $\max$ operation.
Similarly, \cref{lem:bestauc}
suggests two different unbiased estimators 
of the optimal AUC,
namely the min formula
$
  \widehat{\bestauc_1} 
  \coloneqq
  \frac{2}{n(n-1)} \sum_{i<j} 
  \phimin_{\auc}(\eta_{i}, \eta_{j})
$
and the max formula
$
  \widehat{\bestauc_2} 
  \coloneqq
  \frac{2}{n(n-1)} \sum_{i<j} 
  \phimax_{\auc}(\eta_{i}, \eta_{j}) 
$,
where $\sum_{i<j}$ denotes the summation over 
all pairs of indices
$\set{(i, j) \in \{1, \dots, n\}^2 \mid i < j}$.\footnote{
  Naively, $\widehat{\bestauc_1}$ and $\widehat{\bestauc_2}$
  seem to
  require $\Theta(n^{2})$ time to compute
  due to this double summation.
  However, we will show that
  they can be computed in $O(n \log n)$ time
  later in \cref{sec:alg-bestauc}.
}


Thus, a natural question is:
\emph{Which estimator, the min formula or the max formula, is better?}
Two unbiased estimators are usually compared
in terms of their variances;
the one with a smaller variance is considered better
\citep{lehmann1998theory}.
Therefore, we want to be able to guess
which estimator has a smaller variance
for a given data distribution.

To this end, for each of BER and AUC,
we define a \emph{discriminant}
that indicates which estimator,
the min formula or the max formula,
has a smaller variance.
The discriminant for BER is defined as
$\Delta_{\ber} \coloneqq (1 - 2 \theta) \E{ (\eta(x) - \theta) \abs{\eta(x) - \theta}}$.
For AUC, we define
$\Delta_{\auc} \coloneqq (1 - 2 \theta) \E{ (\eta(x) - \theta) \abs{\eta(x) - \eta(x')}}$,
where
$x'$ is an i.i.d.\ copy of $x$.
The following theorem 
suggests that
the sign of each discriminant
can be used to choose the better estimator.


\begin{theorem}[store=thm:min-vs-max:necessary-and-sufficient]~\\\vspace{-2em}
  \label{thm:min-vs-max:necessary-and-sufficient}
  \begin{enumerate}[label=(\roman*)]
    \item 
      For all $n \in \N$, we have 
      $\Var{\widehat{\bestber_1}} \leq \Var{\widehat{\bestber_2}}$ 
      if and only if $\Delta_{\ber} \geq 0$.
    \item
      Assume that the random variable 
      $\eta(x)$ is not a.s.\ constant.
      Then,
      we have $\Var{\widehat{\bestauc_1}} < \Var{\widehat{\bestauc_2}}$
      for all $n \geq 2$
      if and only if $\Delta_{\auc} \geq 0$.
  \end{enumerate}
\end{theorem}

In practice, the discriminants
can be unbiasedly estimated from soft labels as
$
\widehat{\Delta}_{\ber} 
  \coloneqq 
  \frac{1 - 2 \theta}{n} 
  \sum_{i=1}^{n} 
  (\eta_{i} - \theta) \abs{\eta_{i} - \theta}
$
and
$
\widehat{\Delta}_{\auc} 
  \coloneqq 
  \frac{1 - 2 \theta}{n (n - 1)} 
  \sum_{i=1}^n \sum_{j \text{: } j \neq i}
  (\eta_{i} - \theta) \abs{\eta_{i} - \eta_{j}}
$,\footnote{
  Despite the double summation,
  $\widehat{\Delta}_{\auc}$ can be computed in $O(n \log n)$ time
  as shown in 
  \cref{alg:auc-delta-vhat}
  in the appendix.
}
and we can choose between the min formula
and the max formula
based on 
the signs of these estimates, i.e.,
$\sign (\widehat{\Delta}_{\ber})$ 
and
$\sign (\widehat{\Delta}_{\auc})$.\footnote{
  It is also possible to construct
  Wald-type statistical hypothesis tests
  on the signs of $\Delta_{\ber}$ and $\Delta_{\auc}$  
  based on the asymptotic normality of
  $\widehat{\Delta}_{\ber}$ 
  and
  $\widehat{\Delta}_{\auc}$;
  see \cref{sec:proof-clean:discriminants:test}
  for details about the AUC case.
}

Theoretically, 
some sufficient conditions 
can be shown
for $\Delta_{\ber} \geq 0$
and $\Delta_{\auc} \geq 0$,
i.e., the min formulas to be better estimators.
An obvious sufficient condition is
that the two classes are balanced, 
i.e., $\theta = \frac{1}{2}$.
Another condition is that
the Bayes error $\besterr$ is small enough,
or in other words,
the inherent label uncertainty
of the data distribution is sufficiently low.
See \cref{prop:min-vs-max:formal} for
the formal statement and proof.

In the rest of this paper,
our theoretical results are stated
mainly for the min formula estimators
unless explicitly stated otherwise,
and we denote them just by
$\widehat{\bestber}$ and $\widehat{\bestauc}$
for brevity.
However, similar results also hold
for the max formula estimators.


==> sections/clean/ber-auc/unknown-class-prior.tex <==
\subsection{Unknown class prior}
\label{sec:unknown-class-prior}

So far, we have assumed that the class prior
$\theta = \P{y = 1}$
is known.
When the class prior is unknown,
we can still estimate it from the soft labels
simply by the sample mean 
$\bar{\eta} \coloneqq \frac{1}{n} \sum_{i=1}^{n} \eta_{i}$\footnote{
  \citet{jeong2024data} 
  proposed to estimate the class prior by 
  $\frac{1}{n} \sum_{i=1}^{n} \I{\eta_{i} \geq 0.5}$
  in their discussion of the soft-label-based estimation of
  the FPR and FNR of the Bayes optimal classifier
  (i.e., the classifier $h^*(x) = \I{\eta(x) \geq 1/2}$
  that achieves the Bayes error rate $\besterr$).
  However, it is easy to construct examples where
  their estimator becomes biased 
  and statistically inconsistent
  (see \cref{ex:jeong-class-prior-counterexample}).
}
since we have $\E{\eta_{i}} = \theta$.
However, using $\bar{\eta}$ directly in place of $\theta$
in the definitions of 
$\widehat{\bestber}$ 
and 
$\widetilde{\bestauc}$
may cause numerical instability 
or even zero division
since both estimators involve division 
by $\theta$
and $1 - \theta$.
A simple solution to this problem is to
use a clipped version of
$\bar{\eta}$:
$\widehat{\theta}_\epsilon
\coloneqq 
\clip_{\epsilon}^{1 - \epsilon}(\bar{\eta})
=
\min \set{
  1 - \epsilon,
  \max \set{ \epsilon, \bar{\eta} }
}
$,
where
$\epsilon \in (0, \frac{1}{2})$
is some clipping threshold.

With a \emph{fixed} threshold $\epsilon$,
however, 
we must choose $\epsilon$ carefully
so that $0 < \epsilon < \min \set{\theta, 1 - \theta}$;
otherwise,
our clipped estimator $\widehat{\theta}_\epsilon$
and the resulting plug-in estimators
for $\bestber$ and $\bestauc$
will be statistically inconsistent
and
suffer from bias that never vanishes
as $n \to \infty$.
Such a choice of $\epsilon$ requires 
certain prior knowledge of $\theta$.
We can bypass this issue by using
a \emph{vanishing} threshold $\tau_{n}$ 
that depends on the sample size $n$ and tends to zero
as $n$ increases.
For our theoretical analysis,
we set the threshold as follows.

\begin{assumption}[store=ass:unknown-class-prior:epsilon]
  \label{ass:unknown-class-prior:epsilon}
  The clipping threshold is set to 
  $\tau_{n} = \frac{c}{n}$
  for some constant $0 < c < \frac{1}{2}$.
\end{assumption}

The error of the resulting class prior estimator
$\thetahat$
is bounded as follows.

\begin{lemma}[store=lem:unknown-class-prior:bernstein]
  \label{lem:unknown-class-prior:bernstein}
  Under \cref{ass:unknown-class-prior:epsilon},
  for any 
  $\delta > 0$
  and
  $
    n \geq \frac
      {\paren{2 \log (2 / \delta) + 3c}^2}
      {18 \theta (1 - \theta) \log (2 / \delta)}
  $,
  with probability at least $1 - \delta$,
  we have
  $
    \lvert 
      \thetahat - \theta 
    \rvert
    \leq
    \sqrt{\frac{8 \theta (1 - \theta) \log (2 / \delta)}{n}}
  $.
\end{lemma}

We can now estimate $\bestber$ and $\bestauc$
by plugging in $\thetahat$
in place of $\theta$
in the definitions of
$\widehat{\bestber}$
and
$\widetilde{\bestauc}$.
Let us abuse the notation a bit
and denote these plug-in estimators by
$\widehat{\bestber}(\thetahat)$
and
$\widetilde{\bestauc}(\thetahat)$,
respectively.
It can be shown that 
they
are statistically consistent.
More specifically, the following
finite-sample error bounds hold;
see
\cref{thm:unknown-class-prior:ber,thm:unknown-class-prior:auc}
for the proofs.
\begin{theorem}[store=thm:unknown-class-prior:summary]
  \label{thm:unknown-class-prior:summary}
  Under \cref{ass:unknown-class-prior:epsilon},
  for any 
  $\delta > 0$,
  each of the following holds
  with probability at least $1 - \delta$:
  $
    \abs{
      \widehat{\bestber}(\thetahat) - \bestber
    }
    \leq 
    \frac{17}{8}
    \sqrt{
      \frac{2 \log (4/\delta)}{\theta (1 - \theta) n}
    }
  $
  and
  $
    \abs{
      \widetilde{\bestauc}(\thetahat) - \bestauc
    }
    \leq 
    10
    \sqrt{
      \frac{\log (4/\delta)}{\theta (1 - \theta) n}
    }
  $.
\end{theorem}
Also, 
these estimators are asymptotically unbiased;
see \cref{prop:unknown-class-prior:ber-mse,prop:unknown-class-prior:auc-mse}.


==> sections/evaluation/ber-auc.tex <==
The following theorem characterizes the optimal BER and AUC for the noise-injected distribution.

\begin{theorem}[store=thm:feebee]
  \label{thm:feebee}
  For $t \in [0, \frac{1}{2}]$, define
  $
    F_{\nu}(t) \coloneqq
    \frac{
      \lambda_{\nu} \paren{
        2 \theta (1 - \theta) t + \theta^{2}
      }
      - \lambda_{\nu}(\theta)^{2}
    }{
      2 \lambda_{\nu}(\theta) (1 - \lambda_{\nu}(\theta))
    }
  $.
  For any noise level $\nu \in [0, 1)$, 
  the optimal BER and AUC for
  the noise-injected distribution are given by
  $
    \bestber_\nu = F_{\nu}(\bestber)
  $
  and
  $
    \bestauc_\nu = 1 - F_{\nu}(1 - \bestauc)
  $,
  respectively.
\end{theorem}


==> sections/evaluation/bias.tex <==
\paragraph{Bias sensitivity}

Without knowledge of the true optimal BER and AUC values,
another way to assess the quality of an estimator
is to compute the bootstrap variance of the estimator.
However, the bootstrap variance only accounts for the variance of the estimator
and does not reflect the estimator's bias.
By contrast,
our score can reflect certain types of estimator bias;
see \cref{sec:evaluation:bias} for details.
Roughly speaking, any bias larger than the interval width
$U_{\ber}(\nu) - L_{\ber}(\nu)$ produces a positive
penalty in expectation even if the estimator has zero variance.
The interval width scales as $1 - \nu$ and thus approaches zero
as $\nu \to 1$.
Therefore, for example, any constant additive bias that persists across noise levels
is expected to be detected at a sufficiently large noise level.
In this way,
aggregating bound violations over different noise levels
provides a meaningful signal of estimator quality.


==> sections/experiments/estimation.tex <==
\subsection{Estimation on synthetic data}
\label{sec:experiments:estimation}

We first demonstrate the effectiveness of
the proposed estimators by 
a simple experiment with synthetic data.
Similarly to \citet{ushio2025practical},
we draw $n = 10{,}000$ points from 
a two-dimensional Gaussian mixture
with class prior $\theta = 0.2$.
We consider three settings: 
a \emph{clean} one where
the true soft labels $\eta_{i}$ are given,
and two corrupted ones where
the observed corrupted soft labels $\xi_{i}$ 
are either \emph{under-confident} (pulled toward $0.5$)
or \emph{over-confident} (pushed toward $0$ or $1$).
We use
the inverses of beta-calibration maps \citep{kull2017beta}
as the underlying skew functions $f$ 
following \citet{ushio2025practical}.
For each setting and metric, 
we report
the point estimate and 95\% bootstrap confidence interval (CI)
of the proposed estimator, namely,
the estimator of \cref{sec:clean} applied to $\eta_{i}$ 
in the clean setting (\emph{clean}),
and
the estimator of \cref{sec:corrupted} 
based on isotonic regression
in the corrupted settings (\emph{calibrated}).
For the corrupted settings, 
we also report a naive baseline (\emph{raw}) that applies 
$\widehat{\bestber}$ 
or
$\widetilde{\bestauc}$
to the raw, uncalibrated $\xi_{i}$.
In all cases, the class prior $\theta$ is 
treated as unknown and estimated from the data,
as described earlier in \cref{sec:clean,sec:corrupted}.
We use the discriminant-based rules of \cref{sec:min-vs-max}
to pick between the min and max formulae
on each sample.
We also report the ground-truth optimal values,
which can be computed in closed form using \cref{prop:gaussian}
under this Gaussian-mixture setting.

\begin{figure}[t]
  \centering
  \begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/estimation/ber.pdf}
    \caption{BER}
    \label{fig:estimation:ber}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/estimation/auc.pdf}
    \caption{AUC}
    \label{fig:estimation:auc}
  \end{subfigure}
  \caption{
    The estimated optimal BER and AUC values with 95\% bootstrap CIs on synthetic data;
    the dashed lines mark the ground-truth optimal values
    computed in closed form.
  }
  \label{fig:estimation}
\end{figure}

\Cref{fig:estimation} shows the results.
The outputs by the proposed estimators 
(blue bars)
were clustered near 
the ground-truth values (dashed lines)
for both BER and AUC
while the naive baselines
on corrupted soft labels (orange bars)
had deviations an order of magnitude larger than the CI width,
showing that the isotonic calibration of \cref{sec:corrupted}
plays an essential role in correcting the soft label corruption.


==> sections/experiments/max-min.tex <==
\subsection{Real-data experiment: Discriminants and evaluation scores}
\label{sec:experiments:max-min}

We then perform estimation on 
different real-world datasets of soft labels 
from various domains
to support
(i) our discriminant theory in \cref{sec:min-vs-max} and
(ii) our proposed evaluation method in \cref{sec:evaluation}.
Here we only discuss the results for BER (\cref{tab:max-min:ber}),
but the results are qualitatively similar for AUC (\cref{tab:max-min:auc}).
First, on each dataset we tested which of
the min/max formula estimators
had smaller bootstrap variance estimates
and then we compared this with the sign of the empirical discriminants.
The result is shown in the
$\widehat{\Delta}_{\ber}$ and $\Delta \mathrm{SE}$
columns of \cref{tab:max-min:ber},
which aligns well with 
our theory that the sign of the discriminant can
predict which estimator has smaller variance.
The only sign mismatch is on Fashion-MNIST, 
where $\widehat{\Delta}$ is close to zero.

Next, 
we computed our evaluation score for each of the min/max estimators
using the following choices of the parameter $\beta$:
(i) $\beta = 0.5$,
(ii) $\beta = \theta$ (estimated class prior), 
and
(iii) average of the scores $s_{\beta}$
over $\beta \in \{0.1, 0.2, \dots, 0.9\}$,
which are shown on the right side of \cref{tab:max-min:ber}.
We then compared them with the difference of
bootstrapped standard errors.
The results
indicate that
the scores averaged over different $\beta$ values
are far more consistent with
the variance estimates than the scores at individual values
($\beta = 0.5$ or $\beta = \theta$).
Note that this agreement does not imply that our score
can be replaced by bootstrap variance estimates.
As mentioned in \cref{sec:evaluation},
estimator bias can affect our score
even when estimator variance remains unchanged.
Bootstrap variance estimates, in contrast, quantify only estimator variance.

\begin{table}
  \centering
  \footnotesize
  \caption{
    Min vs.\ max formula estimators of
    $\bestber$ and $\bestauc$.
    $\widehat{\Delta}_{\ber}, \widehat{\Delta}_{\auc}$:
    the empirical discriminants $\pm$ its bootstrap standard errors;
    $\Delta\mathrm{SE}$, $\Delta\mathrm{Score}$:
    the $\max - \min$ gaps in
    the bootstrap standard error and evaluation score.
  }
  \begin{subtable}{\linewidth}
    \centering
    \caption{BER}
    \label{tab:max-min:ber}
    \subimport{.}{tables/findings_ber}
  \end{subtable}
  \begin{subtable}{\linewidth}
    \centering
    \caption{AUC}
    \label{tab:max-min:auc}
    \input{sections/experiments/tables/findings_auc.tex}
  \end{subtable}
\end{table}




==> sections/experiments/tables/findings_auc.tex <==
\begin{tabular}{@{}lccccc@{}}
  \toprule
   & & & \multicolumn{3}{c}{$\Delta\mathrm{Score}$} \\
  \cmidrule(l){4-6}
  Dataset & $\widehat{\Delta}_{\auc}$ & $\Delta\mathrm{SE}$ & $\beta = 0.5$ & $\beta = \theta$ & $\beta$ averaged \\
  \midrule
    CIFAR-10 & $+0.0094 \pm 0.0009$ & $+2.08 \times 10^{-4}$ & $-0.0272$ & $-5.34 \times 10^{-4}$ & $+0.4168$ \\
    Fashion-MNIST & $(+0.00 \pm 5.09) \times 10^{-5}$ & $+5.83 \times 10^{-5}$ & $-1.75 \times 10^{-4}$ & $-1.85 \times 10^{-4}$ & $+0.4364$ \\
    SNLI & $+0.0182 \pm 0.0018$ & $+0.0151$ & $-0.2275$ & $-0.0820$ & $+0.1608$ \\
    MNLI & $+0.0091 \pm 0.0014$ & $+0.0144$ & $-0.1951$ & $-0.0503$ & $+0.1773$ \\
    AbductiveNLI & $(+1.10 \pm 2.91) \times 10^{-4}$ & $+3.19 \times 10^{-4}$ & $+7.99 \times 10^{-4}$ & $+0.0012$ & $+0.4303$ \\
    ICLR 2017--2026 & $+0.0076 \pm 0.0002$ & $+0.0011$ & $-0.0048$ & $+0.0530$ & $+0.2072$ \\
  \bottomrule
\end{tabular}


==> sections/experiments/tables/findings_ber.tex <==
\begin{tabular}{@{}lccccc@{}}
  \toprule
   & & & \multicolumn{3}{c}{$\Delta\mathrm{Score}$} \\
  \cmidrule(l){4-6}
  Dataset & $\widehat{\Delta}_{\ber}$ & $\Delta\mathrm{SE}$ & $\beta = 0.5$ & $\beta = \theta$ & $\beta$ averaged \\
  \midrule
    CIFAR-10 & $+0.0093 \pm 0.0009$ & $+2.62 \times 10^{-5}$ & $-0.0068$ & $-2.53 \times 10^{-4}$ & $+0.4236$ \\
    Fashion-MNIST & $(+0.00 \pm 9.12) \times 10^{-5}$ & $-4.03 \times 10^{-5}$ & $+6.76 \times 10^{-5}$ & $+8.71 \times 10^{-5}$ & $+0.4332$ \\
    SNLI & $+0.0136 \pm 0.0023$ & $+0.0044$ & $-0.0545$ & $-0.0319$ & $+0.3868$ \\
    MNLI & $+0.0063 \pm 0.0020$ & $+0.0047$ & $-0.0433$ & $-0.0210$ & $+0.3567$ \\
    AbductiveNLI & $(+1.75 \pm 4.14) \times 10^{-4}$ & $+1.71 \times 10^{-4}$ & $+4.32 \times 10^{-4}$ & $+7.52 \times 10^{-4}$ & $+0.6099$ \\
    ICLR 2017--2026 & $+0.0114 \pm 0.0003$ & $+0.0027$ & $-0.0011$ & $+0.0331$ & $+0.4380$ \\
  \bottomrule
\end{tabular}

